Physics of high energy atmospheric muons

In the first part of the talk the interesting new results of MINOS, OPERA and CMS collaborations (connected with the observational evidence of the rise in the muon charge ratio at muon energies around 1 TeV) are briefly discussed from theoretical point of view. A short review of charge asymmetric effects in muon energy losses is given. In the second part of the talk, the modern theoretical approaches to the problem of heavy quark production in high energy nucleon-nucleus interactions are briefly considered (color dipole formalism, saturation models). The recent new theoretical developments in the ancient problem of intrinsic charm are also discussed.

==> ltpatch.ltx <==

%%%%
%%%% Patch file for the LaTeX2e kernel dated 2009/09/24
%%%% (2009/09/24)

\def\fmtversion@topatch{2009/09/24} % This patch will not work with
                                    % any other release.

\def\patch@level{0}




%%%%%%%%%%%%%%%
\iffalse

\typeout{%
^^J%
*********************************************^^J%
ltpatch.ltx has fixed certain problems with the `kernel' of LaTeX.^^J%
Certain other files in the LaTeX distribution have also been updated^^J%
since the last release (list correct as of 2009/09/24):^^J%
base/xxxxxxx.dtx..............(patch 1)^^J%
unpacked/yyyyyyy.cls..........(patch 1)^^J%
^^J%
See the file patches.txt for more details.^^J%
*********************************************}

\fi

\endinput








